Investigating Pre-trained Audio Encoders in the Low-Resource Condition

Pre-trained speech encoders have been central to pushing state-of-the-art results across various speech understanding and generation tasks. Nonetheless, the capabilities of these encoders in low-resource settings are yet to be thoroughly explored. To address this, we conduct a comprehensive set of experiments using a representative set of 3 state-of-the-art encoders (Wav2vec2, WavLM, Whisper) in the low-resource setting across 7 speech understanding and generation tasks. We provide various quantitative and qualitative analyses on task performance, convergence speed, and representational properties of the encoders. We observe a connection between the pre-training protocols of these encoders and the way in which they capture information in their internal layers. In particular, we observe the Whisper encoder exhibits the greatest low-resource capabilities on content-driven tasks in terms of performance and convergence speed.

==> 6-acknowledgements.tex <==
We would like to thank ISCA and the organising committees of past INTERSPEECH conferences for their help, and praise all our co-authors for their work.

==> intro-backup.tex <==

% \begin{itemize}
%     \item (1p) background
%         \begin{itemize}
%             \item advance in speech is largely drivedn by pre-training
%             \item typical setting: self-supervised pre-training on unlabelled data
%             \item need of a standalone decoder for downstream applications; fine-tuning is required.
%             \item The method is limited, because 
%             \begin{itemize}
%                 \item limited data
%                 \item training complexities (may focus on the lack of mapping)
%                 \item brittleness of pre-trained representations.
%             \end{itemize}
%         \end{itemize}
    
%     \item (1p) introduce Whispter and the gap in the end
%         \begin{itemize}
%             \item The tackle the issues, XX proposed Whisper, which consists of an audio encoder and a text decoder. 
%             \item Pre-trained on massive web-crawled data in a supervised fashion, Whisper naturally learns a mapping between the encoder and decoder and exhibit robust performance on several speech tasks. 
%             \item Its ability to generalise well to held-out datasets on Automatic Speech Recognition (ASR) that it has never seen indicates the high quality of its pre-trained representations.
%             \item Despite this, it remains questions that how Whisper performs on a wider range of speech-tasks.
%             % and how to better use it in practice where data resources are often limited.
%         \end{itemize}

%     \item (1p) Our aim and method 
%         \begin{itemize}
%             \item introduce SUPERB and SUPERB-SG. (These tasks highlight the features of general speech processing tasks: content, speaker, semantics, and enhanced speech processing task: speech translation.)
%             \item In this work, we investigate the capabilities of Whisper in the low resource settings.
%             \item briefly explain why we select these tasks, plus our hypothesis that Whisper captures content.
%             \item Our contributions are in three-folds:
%                 \begin{itemize}
%                     \item run experiments over a wide range of tasks. 
%                     \item analysis 
%                     \item practical guidance.
%                 \end{itemize}
%         \end{itemize}
        


% \end{itemize}


In recent years, the advancement in various speech tasks has largely been driven by encoder models that are typically pre-trained on large-scale datasets via self-supervised learning~\cite{mohamed2022self,DBLP:journals/patterns/LiuMPQJKHS22}. As the prominent examples, the Wav2Vec2~\cite{baevski2020wav2vec} model leverages a speech quantiser module to simulate token prediction of BERT~\cite{kenton2019bert}, while  HuBERT~\cite{hsu2021hubert} adopts a  clustering method to produce discrete labels for each 
% frame (from Michelle: frame is not accurate)
feature vector to imitate masked language model loss. Similar to HuBERT, WavLM~\cite{chen2022wavlm} proposes a denoising masked speech modelling, which masks segments of speech signals to predict the at the output. 

%and subsequently fine-tuned on specific downstream tasks. 
%This has been established as the main paradigm for approaching speech understanding and generation problems. 
%A crucial indicator in evaluating the pre-training process is the ability to generalise, which refers to whether the models can achieve competitive performance on unseen datasets and downstream tasks. A typical adopted strategy to pre-train is utilising massive unlabelled data for self-supervised learning~\cite{hsu2021hubert,chen2022wavlm,baevski2020wav2vec}. 
%in self-supervised tasks so that models can adapt to 
%. Hence, a standalone decoder is required for downstream applications and to leverage the speech representations during fine-tuning. While this strategy is limited: (i) Datasets for specific downstream tasks are limited. However,
%
While it is expected that these pre-trained encoders produce universal speech features effective for a broad range of downstream tasks, in practice pre-trained models still require  large amounts of fine-tuning labelled data to produce state-of-the-art performance, or to converge. This could be attributed to their inefficiency in utilising the representation space~\cite{DBLP:conf/emnlp/YangZHS22}, as well as the difference between the objectives for pre-training and fine-tuning steps~\cite{radford2022robust}. For instance, the pre-training objective is typically designed in the absence of any textual or content cue (i.e., to predict masked speech segments), while the downstream tasks (i.e., automatic speech recognition and speech translation) often require a mapping between speech and text. 
%
%As the prominent examples, the Wav2Vec2~\cite{baevski2020wav2vec} model leverages a speech quantiser module to simulate token prediction of BERT~\cite{kenton2019bert}, while the HuBERT~\cite{hsu2021hubert} adopts a  clustering method to produce discrete labels for each frame to imitate masked language model loss. Similar to HuBERT, WavLM~\cite{chen2022wavlm} proposes a denoising masked speech modelling, which masks segments of speech signals to predict the at the output. 
%WavLM achieves state-of-the-art results on several downstream tasks from SUPERB benchmark~\cite{DBLP:conf/interspeech/YangCCLLLLSCLHT21}.
%
%
%\textcolor{red}{Ehsan: write 3 sentences and summarize the self-supervised learning objective of w2v2, hubert, wavLM. Dedicate 1 sentence per each model.}
%(i.e., often  complexity of self-supervised tasks will likely cause a lack of mapping since none of the downstream task goals is adopted for pre-training. (iii) The brittleness of pre-trained representations. The space of speech representation is easily destroyed in low-resource settings or with disturbance in the data.
%
An exception in this space is the Whisper encoder-decoder model~\cite{radford2022robust}, which leverages weak supervision through large scale crawled data of~(audio, transcript) pairs from the internet, and is pre-trained by learning the mapping between speech and decoder outputs (i.e., in transcription or and translation).
%, allowing it to do zero-shot transfer learning.
%We cover these in more details in Section~\ref{sec:relwork}. 
%
%consisting of an audio encoder and a text encoder, which crawls large-scale data on the Internet for multilingual pre-training under weak supervised conditions. Additionally, prompting is adopted in the decoder to make models learn the map between speech signals and transcriptions, allowing it exhibits robust performance on several speech tasks. Especially the high quality of its pre-trained representations is reflected in its ability to generalise well to held-out datasets on Automatic Speech Recognition (ASR) that it has never seen. 
%
%\textcolor{red}{Ehsan: up-to-here}
%
%, and enhanced speech processing task: speech translation.


To better understand the interplay between pre-training protocols of speech encoders, the amount of fine-tuning data, and speech task types, we conduct a comprehensive study in this work. We evaluate a set of three very recent speech models (Wav2vec2, WavLM, and Whisper) and assess their performance on 7 downstream tasks (covering content, speaker and semantic types) in the low-resource setting. 
%
%
%
%tasks a\textcolor{red}{Ehsan: needs a better transition} \reza{Despite their widespread use, it is understudied how the difference between the pre-training protocols of these encoders translates into representational properties and their downstream performance in the context of tasks which require a varying degree of speaker, semantic, or content information.}\noteRH{It is complex and long; break it to shorter and simpler sentences} 
%\mich{In this work, we investigate this problem in the low-resource scenario where these encoder play a major role in task performance in the absence of sufficiently large data.}
% A particularly interesting setting is the low-resource scenario which places the emphasis on the task solving capabilities of these encoders in the absence of sufficiently large fine-tuning data. 
% To investigate this research question, 
 %
%In this work, content and semantics are considered as content-related tasks. We speculate that \textsc{Whisper} encoders are good at capturing content from speech features.
%
%introduce SUPERB~\cite{DBLP:conf/interspeech/YangCCLLLLSCLHT21} and SUPERB-SG~\cite{tsai2022superb} benchmark covering the performance of widely used pre-trained speech encoders on various downstream tasks. 
%
%nvestigate the capabilities of \textsc{Whisper} encoders to cope with low-resource scenarios, both in terms of performance and convergence speed, and evaluate the quality of the representation space. We 
%
%\textcolor{red}{Ehsan: Need a new paragraph here, summarizing the key experimental findings of the paper. You can highlight: (1) how these encoders do in low-resource setting compared to one another (2-3 sentences), (2) how their performance differ in semantic, content, speaker tasks and how this was related to their pre-training protocols (2-3 sentences), (3) what distinguishing factors they had on the representational properties, e.g. t-SNE or isotropy (2-3 sentences)}
%
%\noteES{Ehsan: Need a new paragraph here, summarizing the key experimental findings of the paper. You can highlight: (1) how these encoders do in low-resource setting compared to one another (2-3 sentences), (2) how their performance differ in semantic, content, speaker tasks and how this was related to their pre-training protocols (2-3 sentences), (3) what distinguishing factors they had on the representational properties, e.g. t-SNE or isotropy (2-3 sentences)}
%\textcolor{blue}{Our experimental findings indicate: (i) Whisper significantly improves the downstream task performance and speedups the convergence in low-resource settings. Compared to baselines, even lightweight versions perform competitively. (ii) Whisper takes advantage in content-related (content, semantics) tasks; however, it is weaker than baselines in the speaker task, which verifies our speculation that weakly supervised pre-training facilitates the capability of capturing the content information in audio. (iii) Whisper notably reshapes the speech representation space. It shows apparent clustering in t-SNE visualisation and dramatically boosts the isotropy score without task-specified fine-tuning.}
Through extensive experiments in the low-resource setting, we found that  Whisper significantly outperforms Wav2ev2 and WavLM by a large margin on content-related (content, semantics) tasks, and shows performance degradation when speaker information is required for a downstream task. To investigate how this behaviour is connected with Whisper's pre-training and representational properties, 
%We hypothese that this is because the pre-training protocol used by Whisper to transform speech input into textual output inherently enhances its ability to capture content. We verify this hypothesis by 
we examine layer-wise information of Whisper and the other baselines. Additionally, through qualitative and quantitative analyses, we highlight how Whisper's superior performance could be attributed to the properties of its representational space. 
%that Whisper notably reshapes the representation space after visualising the space with t-SNE plots. This is also verified by the increase in isotropy score of Whispter over the baselines. 
%
{We hope our study to provide insights for a more effective use of pre-trained speech encoders in the resource-constrained setting.}

% (ii) Whisper takes advantage ; however, it is weaker than baselines in the speaker task, which verifies our speculation that weakly supervised pre-training facilitates the capability of capturing the content information in audio. (iii) Whisper notably reshapes the speech representation space. It shows apparent clustering in t-SNE visualisation and dramatically boosts the isotropy score without task-specified fine-tuning.}


%Our main contributions are:

%\begin{itemize}
 %   \item We conduct experiments with \textsc{Whisper} encoders to evaluate the performance and fine-tuning consumption on a wide range of downstream tasks compared to current advanced pre-trained speech encoders.
%    \item We analyse speech representations generated by \textsc{Whisper} encoders from multiple perspectives and explore the difference between supervision and self-supervision.
 %   \item We provide practical guidance on using \textsc{Whisper} for researchers.
%\end{itemize}
